RMBRec: Robust Multi-Behavior Recommendation towards Target Behaviors

Multi-behavior recommendation faces a critical challenge in practice: auxiliary behaviors (e.g., clicks, carts) are often noisy, weakly correlated, or semantically misaligned with the target behavior (e.g., purchase), which leads to biased preference learning and suboptimal performance. While existing methods attempt to fuse these heterogeneous signals, they inherently lack a principled mechanism to ensure robustness against such behavioral inconsistency. In this work, we propose Robust Multi-Behavior Recommendation towards Target Behaviors (RMBRec), a robust multi-behavior recommendation framework grounded in an information-theoretic robustness principle. We interpret robustness as a joint process of maximizing predictive information while minimizing its variance across heterogeneous behavioral environments. Under this perspective, the Representation Robustness Module (RRM) enhances local semantic consistency by maximizing the mutual information between users' auxiliary and target representations, whereas the Optimization Robustness Module (ORM) enforces global stability by minimizing the variance of predictive risks across behaviors, which is an efficient approximation to invariant risk minimization. This local-global collaboration bridges representation purification and optimization invariance in a theoretically coherent way. Extensive experiments on three real-world datasets demonstrate that RMBRec not only outperforms state-of-the-art methods in accuracy but also maintains remarkable stability under various noise perturbations. For reproducibility, our code is available at https://github.com/miaomiao-cai2/RMBRec/.

==> temp.tex <==
% \section{Conclusion}

% In this paper, we addressed the critical challenge of behavioral misalignment and noise in multi-behavior recommendation. Unlike prior studies that primarily rely on heuristic fusion strategies, we proposed~\shortname, a target-centric framework that achieves robustness through a \textit{local–global collaborative mechanism}: it aligns behavior representations locally to ensure semantic consistency, while stabilizing optimization globally across heterogeneous behavioral environments. In particular, the \textbf{Representation Robustness Module (RRM)}, which enforces \textit{local semantic consistency} via target-anchored contrastive alignment, and the \textbf{Optimization Robustness Module (ORM)}, which ensures \textit{global optimization stability} by learning invariant user preferences across heterogeneous behavioral environments. Extensive experiments on three real-world datasets demonstrated that~\shortname~consistently outperforms state-of-the-art baselines in both accuracy and robustness, particularly under noisy or misaligned conditions. Furthermore, the proposed \textbf{Behavioral Alignment Ratio (BAR)} provides a simple yet powerful diagnostic perspective for understanding the consistency and reliability of auxiliary behaviors, offering new insights for robustness-aware model design. 

% \begin{itemize}[leftmargin=0.5cm, itemindent=0cm]
    
%     \item \textbf{The effect of invariance regularization is closely tied to dataset characteristics}. On the Beibei dataset, removing invariance regularization results in only a marginal decline in performance, which aligns with its high $Behavioral~Alignment~Ratio \\(BAR)$ values (view: 0.9756, cart: 0.9731). This indicates that auxiliary and target behaviors are already highly consistent, leaving little room for further robustness gains. In contrast, the Tmall dataset exhibits an extremely low $BAR$ for add-to-cart (0.0012), reflecting severe semantic misalignment between cart and purchase. In such noisy environments, invariance regularization produces substantial improvements by preventing the model from overfitting to spurious auxiliary patterns. This highlights the \textbf{dataset-dependent role of invariance regularization}: it provides only minor benefits when auxiliary behaviors are already well aligned (as in Beibei), but becomes critical in noisier datasets like Taobao and TMall, where it significantly enhances robustness.

%     \item \textbf{Removing auxiliary behaviors leads to significant performance drops}, confirming that heterogeneous interactions provide complementary information beyond the target behavior alone. For example, on Taobao, removing \textit{view} decreases HR@10 from 0.1445 to 0.1093 (a 24.3\% drop), and on Beibei, eliminating \textit{add-to-cart} reduces HR@10 from 0.1281 to 0.0793 (a 38.1\% drop). These results clearly demonstrate that \textbf{auxiliary behaviors play an essential role in enhancing recommendation quality}. 
        
%     \item \textbf{The effectiveness of auxiliary behaviors depends on dataset characteristics}. On Beibei, with high $BAR$ values (view: 0.9756, cart: 0.9731), removing cart causes a sharp HR@10 drop of 38.1\%, reflecting strong reliance on auxiliary signals. \textbf{In contrast, TMall is dominated by noise}: its add-to-cart $BAR$ is only 0.0012, meaning almost no overlap with purchases, and removing add-to-cart even improves HR@10 by 22.3\%. These results confirm that well-aligned behaviors boost performance, while nearly pure-noise behaviors harm learning and may cause negative transfer.

%     \item Across all ablation settings, we observe that the complete ~\shortname consistently surpasses its variants in most cases, demonstrating \textbf{the necessity of both alignment modules and auxiliary signals}. In addition, our proposed $BAR$ proves to be a powerful diagnostic tool for characterizing dataset properties: high $BAR$ values (e.g., Beibei) explain why auxiliary behaviors strongly support the target, whereas extremely low $BAR$ values (e.g., TMall add-to-cart = 0.0012) reveal that noisy signals may harm learning if not properly aligned. These findings not only validate the effectiveness of our model design but also emphasize a broader insight: \textbf{understanding dataset-specific behavioral alignment is crucial for building robust multi-behavior recommenders}.
    
% \end{itemize}


% \begin{itemize}[leftmargin=0.5cm, itemindent=0cm]

%     \item \textbf{The relative improvement of ~\shortname~ on Beibei is smaller than on TMall or Taobao}. This is because Beibei has been heavily preprocessed to enforce a strict \textit{view → add-to-cart → buy} chain, leading to highly consistent auxiliary and target behaviors with little noise or drift. In contrast, Taobao shows the highest proportion of direct target, and TMall exhibits extremely low $BAR$ values (e.g., add-to-cart = 0.0012), both of which indicate more severe preference shifts and noisier auxiliary interactions. The substantial gains of ~\shortname~ on these datasets demonstrate that our invariance-based alignment is particularly effective under noisy and misaligned conditions, where it suppresses spurious signals and enhances robustness. 

%     \item We find that \textbf{UIPL does not consistently outperform earlier multi-behavior methods}. For instance, on Beibei, its performance even falls behind MBGCN and PKEF on NDCG@10, suggesting that when auxiliary and target behaviors are already well aligned (high BAR), the VAE-based invariance in UIPL provides little benefit. More importantly, on noisy datasets like TMall, where invariance should have been advantageous, our ~\shortname~ reaches 0.1549 (+4.38\%). This gap reveals a key insight: generative constraints alone cannot effectively capture invariance in multi-behavior settings. By contrast, our framework leverages different behaviors as natural environments, making the invariance regularization more grounded and effective. This design ensures that ~\shortname~ can robustly suppress noise and adapt to diverse dataset characteristics. 

%     \item Compared with multi-behavior approaches, \textbf{single-behavior models consistently yield much weaker performance} across all datasets, highlighting the limitations of relying solely on the target interactions. This gap clearly demonstrates the effectiveness of leveraging auxiliary behaviors to enrich user preference modeling. For instance, on the Beibei dataset, our model outperforms SimGCL—the strongest single-behavior baseline—by +205\% on HR@10 and +222\% on NDCG@10. Such remarkable improvements are largely attributed to Beibei’s high $BAR$, where auxiliary signals (view and cart) are highly consistent with purchases. These results confirm that auxiliary behaviors, when well aligned, provide essential complementary cues that significantly enhance recommendation accuracy beyond what single-behavior methods can achieve. 
    
% \end{itemize}

% We compare ~\shortname ~ with representative baselines from two categories: single-behavior methods and multi-behavior methods.

% \textbf{Single-behavior Model:}
% \begin{itemize}[leftmargin=0.5cm, itemindent=0cm]
%     \item \textbf{LightGCN}~\cite{}: A simplified graph-based model that removes feature transformation and non-linearities, effectively capturing high-order collaborative signals on user–item graphs.
%     \item \textbf{SimGCL}~\cite{Yu2021AreGA}: A contrastive extension of LightGCN that introduces random embedding perturbations with InfoNCE loss, enhancing robustness and representation learning.
% \end{itemize}

% \textbf{Multi-behavior Model:}
% \begin{itemize}[leftmargin=0.5cm, itemindent=0cm]
%     \item \textbf{MBGCN}~\cite{jin2020multi}: A GCN-based multi-behavior model that constructs a unified heterogeneous graph, learns user–item preferences while weighting different behaviors, and incorporates item–item relations to enhance behavior semantics.
%     \item \textbf{CRGCN}~\cite{CRGCN}: A cascading residual GCN that sequentially propagates embeddings across behaviors, progressively refining user preferences, while adopting multi-task learning to jointly optimize target and auxiliary behaviors.
%     \item \textbf{MB-CGCN}~\cite{cheng2023multi}: An extension of CRGCN that refines cascading propagation by simplifying residual connections and aggregating user preferences across all behaviors for more effective target recommendation.
%     \item \textbf{PKEF}~\cite{meng2023parallel}: A parallel knowledge fusion framework with a disentangled multi-expert network, designed to balance heterogeneous behavior distributions and mitigate negative transfer in multi-behavior recommendation.
%     \item \textbf{BCIPM}~\cite{yan2024behavior}: A behavior-contextualized item preference model that leverages auxiliary interactions to enhance target recommendations while suppressing noise from irrelevant behaviors.
%     \item \textbf{S-MBRec}~\cite{gu2022self}: A self-supervised multi-behavior model that tackles the sparsity of target supervision by constructing auxiliary contrastive tasks. It adopts a star-shaped design and provides additional training signals without modeling cross-auxiliary dependencies. 
%     \item \textbf{MBSSL}~\cite{xu2023multi}: A recent self-supervised model that enhances multi-behavior recommendation by applying inter- and intra-behavior contrastive learning. It further introduces an adaptive gradient strategy to balance supervised and self-supervised objectives. 
%     \item \textbf{UIPL}~\cite{yan2025user}: The first attempt to introduce invariant risk minimization into multi-behavior recommendation. It treats each behavior (or combinations thereof) as an environment and applies a VAE-based formulation to impose invariance constraints. However, its reliance on synthetic environments and simplified assumptions limits its ability to capture realistic behavior heterogeneity.  
% \end{itemize}
%%%这是第一个版本，接下来我要写第二个版本，放在附录的一个版本
% We compare~\shortname~with a comprehensive set of representative baselines from two major categories: \textbf{single-behavior models} and \textbf{multi-behavior models}. 
% The former capture user preferences solely from target interactions, while the latter explicitly leverage auxiliary behaviors for enhanced supervision. 
% We further include several recent robustness-oriented methods that explicitly mitigate noisy or inconsistent behaviors, allowing direct comparison with~\shortname~in terms of robustness and stability.
% \noindent\textbf{Single-behavior Models.}
% \begin{itemize}[leftmargin=0.5cm, itemindent=0cm]

%     \item \textbf{LightGCN}~\cite{}: A simplified graph-based collaborative filtering model that removes feature transformation and non-linear activations, effectively capturing high-order user–item relations on the interaction graph.
    
%     \item \textbf{SimGCL}~\cite{Yu2021AreGA}: It introduces random embedding perturbations and an InfoNCE-based regularization. This enhances representation robustness and generalization, making it a strong baseline for robustness comparison.
    
% \end{itemize}

% \noindent\textbf{Multi-behavior Models.}

% \begin{itemize}[leftmargin=0.5cm, itemindent=0cm]

%     \item \textbf{MBGCN}~\cite{jin2020multi}: It constructs a unified heterogeneous graph and adaptively weights different behaviors to learn comprehensive user–item representations.
    
%     \item \textbf{CRGCN}~\cite{CRGCN}: It propagates embeddings across behaviors in sequence, refining user preferences through multi-task learning that jointly optimizes auxiliary and target tasks.
    
%     \item \textbf{MB-CGCN}~\cite{cheng2023multi}: It simplifies residual propagation and aggregates embeddings across all behaviors to strengthen target recommendation.
    
%     \item \textbf{PKEF}~\cite{meng2023parallel}: It is a parallel knowledge fusion framework that employs a disentangled multi-expert structure to balance heterogeneous behavior distributions and reduce negative transfer effects.
    
%     \item \textbf{BCIPM}~\cite{yan2024behavior}: It is a behavior-contextualized item preference model that leverages auxiliary interactions to enhance target recommendation while filtering out noise from irrelevant behaviors.
    
%     \item \textbf{S-MBRec}~\cite{gu2022self}: It alleviates target sparsity by introducing auxiliary contrastive objectives. It adopts a star-shaped design that provides additional training signals without explicitly modeling inter-auxiliary dependencies.
    
%     \item \textbf{MBSSL}~\cite{xu2023multi}: It employs both inter- and intra-behavior contrastive learning to enhance semantic consistency. It further adopts adaptive gradient balancing to maintain stable optimization, thus improving robustness.
    
%     \item \textbf{UIPL}~\cite{yan2025user}: It is the first attempt to incorporate invariant risk minimization into multi-behavior recommendation. It applies a VAE-based invariance constraint. However, its synthetic environment design limits its ability to capture realistic behavioral heterogeneity.
    
% \end{itemize}


% To evaluate the effectiveness of our proposed approach, we conduct experiments on three large-scale e-commerce datasets, namely \textbf{Tmall}~\footnote{}, \textbf{Taobao}~\footnote{}, and \textbf{Beibei}~\footnote{}. These datasets are widely used in multi-behavior recommendation since they naturally include heterogeneous implicit feedback that reflects different stages of user decision-making. In all cases, \textbf{purchase} is regarded as the target behavior, while the remaining interactions (e.g., view, add-to-cart, collect) serve as auxiliary signals. Following established practices in prior research~\cite{}, we retain only the earliest occurrence of each user–item interaction to remove redundant records. 
% The detailed statistics after preprocessing are summarized in Table~\ref{tab:dataset}. 
% \begin{itemize}[leftmargin=0.5cm, itemindent=0cm]
%     \item \textbf{Tmall.} This dataset is collected from Tmall, one of the largest online marketplaces in China. It covers four types of behaviors, including view, collect, add-to-cart, and purchase. 
%     \item \textbf{Taobao.} This dataset is obtained from a widely used Chinese e-commerce platform. It records multiple types of user behaviors, including view, add-to-cart, and purchase. 
%     \item \textbf{Beibei.} This dataset is collected from Beibei, an e-commerce platform specializing in maternal and infant products. It contains three types of interactions, including view, add-to-cart, and purchase. 
% \end{itemize}


% To address this issue, we propose the \textbf{Representation Robustness Module (RRM)}, which enforces \textit{local semantic consistency} across behaviors through a target-anchored contrastive objective. The core is that the target behavior reflects the most trustworthy expression of user preference, while auxiliary behaviors are potentially noisy observations of the same underlying intent. Therefore, rather than directly fusing heterogeneous embeddings, RRM explicitly purifies auxiliary representations by aligning them with the target behavior before aggregation. This \textit{purify-then-fuse} strategy ensures that the resulting user representation is constructed from semantically consistent signals and becomes inherently more robust against spurious or misaligned auxiliary feedback at the representation level. 

% \section{Preliminary}



% Let $\mathcal{U}$ and $\mathcal{I}$ denote the sets of users and items, respectively. Each user $u \in \mathcal{U}$ may interact with item $i \in \mathcal{I}$ through multiple types of behaviors $\mathcal{B} = \{\text{view}, \text{collect}, \text{add-to-cart}, \text{purchase}, \ldots\}$. For each behavior $b \in \mathcal{B}$, we denote the corresponding interaction matrix as $\mathbf{R}^{(b)} \in \{0,1\}^{|\mathcal{U}| \times |\mathcal{I}|}$, where $\mathbf{R}^{(b)}_{u,i} = 1$ if user $u$ has interacted with item $i$ under behavior $b$, and $\mathbf{R}^{(b)}_{u,i} = 0$ otherwise.  

% To model user preferences and item characteristics, we embed users and items into a $d$-dimensional latent space. 
% For each behavior $b \in \mathcal{B}$, we learn behavior-specific user and item embedding matrices $\mathbf{P}^{(b)} \in \mathbb{R}^{|\mathcal{U}| \times d}$ and $\mathbf{Q}^{(b)} \in \mathbb{R}^{|\mathcal{I}| \times d}$, where $\mathbf{p}_u^{(b)}$ and $\mathbf{q}_i^{(b)}$ denote the embeddings of user $u$ and item $i$ under behavior $b$. This formulation enables the model to capture heterogeneous semantics across different types of interactions. 
% To obtain unified representations, we fuse the behavior-specific embeddings via a function $f(\cdot)$:
% \begin{equation}
%     \mathbf{z}_u = f\big(\{\mathbf{p}_u^{(b)} \mid b \in \mathcal{B}\}\big), \quad
%     \mathbf{z}_i = f\big(\{\mathbf{q}_i^{(b)} \mid b \in \mathcal{B}\}\big),
% \end{equation}
% where $\mathbf{z}_u$ and $\mathbf{z}_i$ represent the final user and item embeddings.

% For optimization, we define the predicted preference score as $s(u,i) = \mathbf{z}_u^\top \mathbf{z}_i$. 
% Following common practice in implicit-feedback recommendation ~\cite{He2020LightGCNSA,Rendle2009BPRBP,Koren2009MatrixFT}, we adopt the Bayesian Personalized Ranking (BPR) loss ~\cite{Rendle2009BPRBP} to train the model. Let $\mathcal{O}^+ = \{ (u,i,j) \mid \mathbf{R}^{(\text{target})}_{u,i}=1, \ \mathbf{R}^{(\text{target})}_{u,j}=0 \}$ denote the set of training triplets, where $(u,i)$ is an observed target interaction (e.g., purchase) and $j$ is a negative item unobserved under the target behavior. 
% The loss function is formulated as:
% \begin{equation}
%     \mathcal{L}_{\text{BPR}}^{main} = - \frac{1}{|\mathcal{O^+}|}\sum_{(u,i,j) \in \mathcal{O^+}} \log \sigma \big( s(u,i) - s(u,j) \big)+\lambda\|\Theta\|_2^2,
% \end{equation}
% where $\sigma(\cdot)$ is the sigmoid function and $\Theta$ denotes all trainable parameters.
% Notably, optimization is performed under the \textbf{target behavior} (e.g., purchase), while auxiliary behaviors influence learning indirectly through their contribution to the fused embeddings.


% To better understand the source of inconsistency across behaviors, we propose a simple yet effective diagnostic metric—the \textbf{Behavioral Alignment Ratio (BAR)}—which explicitly centers on the target behavior. Traditional conversion rates typically measure how likely users are to perform the target behavior given an auxiliary action (e.g., the probability of purchase after viewing or adding to cart), reflecting $P(target|auxiliary)$. In contrast, BAR captures the inverse relationship: it quantifies how many target interactions are also accompanied by a particular auxiliary behavior, corresponding to $P(auxiliary|target)$. This target-oriented formulation provides a more direct and robust way to assess how strongly each auxiliary behavior aligns with the objective of target behavior prediction. The detailed definition of BAR is provided in Eqn.~\ref{eq:bar}. 
% Our analysis based on BAR reveals striking differences across datasets. In \textit{Beibei}, BAR values are extremely high (e.g., view = 0.9756), indicating that purchases almost always follow auxiliary actions, suggesting a highly consistent and low-noise environment. In contrast, in \textit{TMall}, the BAR for add-to-cart is as low as 0.0012, implying that such signals are nearly pure noise and contribute little to target prediction. These findings uncover an important insight: auxiliary behaviors differ drastically in their alignment with the target behavior. 
% \textbf{This empirical observation directly motivates our robustness-oriented design: a reliable model must exploit well-aligned signals while resisting noisy or misaligned ones.}

% Most existing studies usually adopt the fusion-based paradigm, which first learns behavior-specific representations and then aggregates them into a unified embedding for prediction, typically through concatenation~\cite{}, multilayer perceptrons (MLPs)~\cite{}, or attention mechanisms~\cite{}. However, in practice, auxiliary interactions are far from clean. Many users casually browse or add items to their carts without genuine intent to purchase, resulting in inconsistent or even misleading supervision signals~\cite{}. Such noisy or weakly correlated behaviors distort the learned user preference space and cause the model to overfit spurious patterns rather than true purchasing intent. As a result, the robustness of multi-behavior recommenders becomes severely compromised in real-world scenarios.

% To alleviate these problems, previous studies have made various attempts from different perspectives. For example, adaptive weighting strategies~\cite{}  and mixture-of-experts networks~\cite{} have been proposed to down-weight unreliable signals, contrastive learning~\cite{khosla2020supervised,wang2020understanding,yang2023generative,Wu2020SelfsupervisedGL} has been introduced to enforce representation consistency~\cite{}, and noise-aware mechanisms have been designed to prune unreliable or spurious interactions~\cite{}. 
% While these approaches achieve partial improvements, they largely rely on heuristic designs or behavior-specific assumptions, and their performance often degrades when auxiliary behaviors are noisy or distributionally biased. In particular, existing methods lack a unified and principled mechanism that can inherently enhance the model’s robustness without relying on explicit noise labels or handcrafted weighting schemes. 
% These limitations highlight a critical gap in existing research: the prevailing fusion paradigm itself is inherently vulnerable to behavioral misalignment and noise. This calls for a paradigm shift from simply fusing all signals to selectively aligning and stabilizing the learning process with the target behavior as the anchor. 


% To quantify such inconsistency, we further propose a simple diagnostic metric, the Behavioral Alignment Ratio (BAR), which measures how strongly each auxiliary behavior aligns with the target one. Empirical analysis reveals large cross-dataset disparities, confirming that auxiliary signals vary widely in their reliability.
% This empirical observation directly motivates our robustness-oriented design: \textbf{\textit{a reliable model must exploit well-aligned signals while resisting noisy or misaligned ones.}}
%\&begin{table*}[t]
% \small
% \centering
% \caption{Overall performance comparison in terms of HR@K and NDCG@K, where $K=10$ and $K=20$. The best results are highlighted in \textbf{bold}, and the second-best are \underline{underlined}. Results marked with * indicate statistical significance with $p$-value $<$ 0.05 over the best baseline (paired t-test).}
% \label{tab:overall}
% \resizebox{\linewidth}{!}{\begin{tabular}{l|l|cc|cccccccc|cc}
% \toprule
% \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metric}} 
% & \multicolumn{2}{c|}{\textbf{Single-Behavior Models}} 
% & \multicolumn{8}{c|}{\textbf{Multi-Behavior Models}} 
% & \multicolumn{2}{c}{\textbf{Ours}} \\
% \cmidrule(r){3-14} 
% & & \textbf{LightGCN} & \textbf{SimGCL} 
%   & MBGCN&\textbf{CRGCN} & \textbf{MB-CGCN} & \textbf{PKEF} & \textbf{BCIPM} & \textbf{S-MBRec} & \textbf{MBSSL} & \textbf{UIPL} & \textbf{\shortname} &  \textbf{\textit{Imp.}}\\
% \midrule
% \multirow{4}{*}{\textbf{Taobao}}  
%  & \textbf{HR@10}   &0.0253 &0.0400 &0.0433 &0.1142 &0.0989 &0.1098 &\underline{0.1257} &0.0568 &0.0861 &0.1225 &\textbf{0.1462*} &\textbf{16.3\%} \\
%  & \textbf{NDCG@10} &0.0137 &0.0236 &0.0263 &0.0632 &0.0471 &0.0627 &0.0708 &0.0328 &0.0480 &\underline{0.0748} &\textbf{0.0969*} &\textbf{29.5\%} \\
%  & \textbf{HR@20}   &0.0364 &0.0522 &0.0811 &0.1477 &0.1368 &0.1223 &\underline{0.1723} &0.0891 &0.1247 &0.1567 &\textbf{0.1766*} &\textbf{2.5\%} \\
%  & \textbf{NDCG@20} &0.0178 &0.0265 &0.0355 &0.0773 &0.0595 &0.0651 &0.0833 &0.0411 &0.0579 &\underline{0.0834}   &\textbf{0.1046*} &\textbf{25.4\%} \\
% \midrule
% \multirow{4}{*}{\textbf{TMall}}  
%  & \textbf{HR@10}   &0.0379 &0.0709 &0.0549 &0.0840 &0.1083 &0.1138 &0.1418 &0.0694 &0.0760 &\underline{0.1484} &\textbf{0.1549*} &\textbf{4.3\%} \\
%  & \textbf{NDCG@10} &0.0205 &0.0399 &0.0285 &0.0442 &0.0426 &0.0642 &0.0743 &0.0362 &0.0421 &\underline{0.0819} &\textbf{0.0838*} &\textbf{2.3\%} \\
%  & \textbf{HR@20}   &0.0486 &0.1018 &0.0799 &0.1238 &0.1370 &0.1676 &\underline{0.2025} &0.1009 &0.1113 &0.2005 &\textbf{0.2132*} &\textbf{5.2\%} \\
%  & \textbf{NDCG@20} &0.0231 &0.0487 &0.0345 &0.0540 &0.0523 &0.0562 &0.0891 &0.0438 &0.0509 &\underline{0.0946} &\textbf{0.0982*} &\textbf{3.8\%} \\
% \midrule
% \multirow{4}{*}{\textbf{Beibei}}  
%  & \textbf{HR@10}   &0.0383 &0.0420 &0.0373 &0.0539 &0.0579 &\underline{0.1130} &0.0670 &0.0489 &0.0626 &0.0693 &\textbf{0.1281*} &\textbf{13.4\%} \\
%  & \textbf{NDCG@10} &0.0207 &0.0210 &0.0198 &0.0259 &0.0381 &\underline{0.0582} &0.0331 &0.0253 &0.0352 &0.0347 &\textbf{0.0676*} &\textbf{16.2\%} \\
%  & \textbf{HR@20}   &0.0607 &0.0665 &0.0639 &0.0944 &0.1073 &\underline{0.1687} &0.1014 &0.0770 &0.0935   &0.1131   &\textbf{0.1882*} &\textbf{11.6\%} \\
%  & \textbf{NDCG@20} &0.0262 &0.0273 &0.0259 &0.0361 &0.0428 &\underline{0.0731} &0.0451 &0.0324 &0.0419   &0.0482   &\textbf{0.0826*} &\textbf{12.9\%} \\
% \bottomrule
% \end{tabular}}
% \end{table*}


 % \item  \textbf{Significant robustness gains under moderate noise.} The most significant improvements are observed on \textit{Taobao}, where auxiliary behaviors are moderately aligned yet noisy. ~\shortname~outperforms the strongest baseline by up to +29.5\% on NDCG@10, confirming that the synergy between RRM’s local alignment and ORM’s global invariance enables the model to effectively filter spurious auxiliary cues while preserving informative signals. 
    
 %    \item  \textbf{Stable performance under extreme misalignment.} On \textit{TMall}, where auxiliary behaviors (e.g., \textit{add-to-cart}) are nearly uncorrelated with purchases ( $BAR \approx  0$ ), ~\shortname ~ still achieves small but consistent gains over the best baseline. This demonstrates that even when auxiliary data is highly noisy, our local–global collaborative design prevents performance degradation. The advantage that most fusion-based or heuristic weighting methods fail to provide. 
    
 %    \item \textbf{Strong performance in well-aligned scenarios.} On \textit{Beibei}, where auxiliary behaviors follow a clean sequential chain (\textit{view} → \textit{cart} → \textit{purchase}), all methods perform well, but ~\shortname~still achieves noticeable gains (e.g., +13.4\% HR@10). Interestingly, PKEF performs competitively here because its multi-expert fusion assumes ordered, semantically coherent behaviors, an inductive bias well-suited to Beibei’s clean interaction patterns. In contrast, ~\shortname~remains consistently robust across datasets without relying on such strict behavioral assumptions. 

We further investigate the sensitivity of the two key hyperparameters in~\shortname: $\lambda_{1}$ and $\lambda_{2}$, which control the weights of the contrastive alignment loss and the invariance regularization term, respectively. These parameters determine the relative importance of enforcing \textit{local semantic consistency} at the representation level and \textit{global optimization stability } across behavioral environments at the optimization level. To examine their effects, we vary $\lambda_{1}$ and $\lambda_{2}$ over a wide range on three datasets, and report the results in Figure~\ref{fig:hyper}. 

Across all datasets, the results exhibit a consistent trend. As the weights increase from small values, model performance first improves, demonstrating that both contrastive alignment and invariance regularization contribute positively to capturing target-oriented semantics and suppressing behavior-specific noise. This validates the effectiveness of~\shortname’s dual-level design, where RRM and ORM collaboratively enhance robustness by aligning auxiliary behaviors locally and stabilizing learning globally. 

However, when the weights become excessively large, performance begins to decline, as the auxiliary objectives start to dominate the main recommendation loss and hurt preference learning. These results suggest that robustness in multi-behavior recommendation does not arise from maximizing auxiliary constraints unconditionally, but from achieving a balanced integration between local alignment and global invariance. 


